How Does Knowledge Selection Help Retrieval Augmented Generation?

Retrieval-augmented generation (RAG) is a powerful method for enhancing natural language generation by integrating external knowledge into a model's output. While prior work has demonstrated the importance of improving knowledge retrieval for boosting generation quality, the role of knowledge selection, a.k.a. reranking or filtering, remains less clear. This paper empirically analyzes how knowledge selection influences downstream generation performance in RAG systems. By simulating different retrieval and selection conditions through a controlled mixture of gold and distractor knowledge, we assess the impact of these factors on generation outcomes. Our findings indicate that the downstream generator model's capability, as well as the complexity of the task and dataset, significantly influence the impact of knowledge selection on the overall RAG system performance. In typical scenarios, improving the knowledge recall score is key to enhancing generation outcomes, with the knowledge selector providing limited benefit when a strong generator model is used on clear, well-defined tasks. For weaker generator models or more ambiguous tasks and datasets, the knowledge F1 score becomes a critical factor, and the knowledge selector plays a more prominent role in improving overall performance.

==> top3_fixed_recall_precision_vs_answer_f1.tex <==
% This plot is wrong!!!! It should not be visualized!
\iffalse
\begin{figure*}
\centering
    \begin{subfigure}[b]{0.48\textwidth}
     \centering
     \includegraphics[width=\textwidth]{GPT-4o-mini_top3_WoW_figures/fixed_recall_precision_vs_answer_f1.pdf}
    %\vspace{-0.5em}
    %  \caption{Contour of Wizard of Wikipedia GPT-4o-mini response F1 versus the knowledge precision score given different knowledge recall scores.} 
    \label{fig:wow_gpt_fixed_recall_precision_vs_answer_f1_k=3}
    \vspace{-1.5em} 
    \end{subfigure}
    \quad
    \begin{subfigure}[b]{0.48\textwidth}
     \centering
     \includegraphics[width=\textwidth]{GPT-4o-mini_top3_HotpotQA_figures/fixed_recall_precision_vs_answer_f1.pdf}
    %\vspace{-0.5em}
    %\caption{Contour of HotpotQA GPT-4o-mini answer F1 versus the knowledge precision score given different knowledge recall scores.} 
    \label{fig:hotpot_qa_gpt_fixed_recall_precision_vs_answer_f1_k=3}
    \vspace{-1.5em} 
    \end{subfigure}
    \quad
    
%\vspace{-1.5em}
\caption{Color contours of answer F1 versus the knowledge precision for GPT-4o-mini on Wizard of Wikipedia (left) and HotpotQA (right) by limiting the number of knowledge sentences up to k=3. Each contour represents a different knowledge recall score; moving left to right visualizes improving the performance (precision) of the knowledge selector. \textit{Each figure is a meta-experiment, and each data point corresponds to a full experiment on the entire sampled dataset.}}
\label{fig:gpt_fixed_recall_precision_vs_answer_f1_k=3}
\end{figure*}
\fi
